First measurement of GaAs as a scintillating calorimeter: achievements and prospects

In this paper we present the first measurement of a Gallium Arsenide (GaAs) crystal as a scintillating calorimeter with dual heat and light readout within the DAREDEVIL project. The experimental setup features a 4.3 g GaAs (GaAs-1) crystal, operated at approximately 10 mK coupled with a Neutron Transmutation Doped (NTD) thermal sensor for phonon detection and an auxiliary calorimeter for the detection of scintillation light. For the GaAs-1 crystal, a baseline resolution of 121$\pm$ 2 eV has been achieved. While, with a 3.5 g GaAs (GaAs-2) crystal an even better baseline resolution of 44.5 $\pm$ 0.8 eV was achieved. Alpha and X-ray calibration sources were used to study the scintillation light response to different types of interacting radiation. The GaAs crystal exhibits a strong particle discrimination capability based on the emitted scintillation light, featuring a light yield (LY) of 0.9 $\pm$ 0.2 keV/MeV for $\alpha$ induced events and 0.07 $\pm$ 0.01 keV/MeV for $\beta$/$\gamma$ events, both measured at 1~MeV. The unusual luminescence behavior, i.e. more light being produced under irradiation by $\alpha$ particles warrants further investigation, particularly due to its potential to enhance sensitivity to low-energy nuclear recoils from light dark matter scattering.

==> Makefile <==
# input
MAIN					= main

MAIN_TEX				= ${MAIN}.tex
MAIN_PDF				= ${MAIN}.pdf

BIBLIOGRAPHY		= ref.bib

# clean
FILE_CLEAN			= *.aux *.bbl *.blg *.brf *.idx *.ilg *.ind *.log *.out *~ *Notes.bib
FILE_DISTCLEAN		= ${MAIN_PDF} ${OUTPUT_PDF}

.PHONY:	pdf biblio \
			rename \
			distclean clean

pdf:	${MAIN_TEX}
	pdflatex ${MAIN}
	evince ${MAIN_PDF}
	
biblio: ${MAIN_TEX} ${BIBLIOGRAPHY} 
	pdflatex ${MAIN}
	bibtex ${MAIN}
#	makeindex ${MAIN}
	pdflatex ${MAIN}
	pdflatex ${MAIN}
	evince ${MAIN_PDF}
	
view:	${MAIN_PDF}
	evince ${MAIN_PDF}
	
distclean:	clean
	rm -f ${FILE_DISTCLEAN}

clean:
	rm -f ${FILE_CLEAN}

